PSDR-Room: Single Photo to Scene using Differentiable Rendering

A 3D digital scene contains many components: lights, materials and geometries, interacting to reach the desired appearance. Staging such a scene is time-consuming and requires both artistic and technical skills. In this work, we propose PSDR-Room, a system allowing to optimize lighting as well as the pose and materials of individual objects to match a target image of a room scene, with minimal user input. To this end, we leverage a recent path-space differentiable rendering approach that provides unbiased gradients of the rendering with respect to geometry, lighting, and procedural materials, allowing us to optimize all of these components using gradient descent to visually match the input photo appearance. We use recent single-image scene understanding methods to initialize the optimization and search for appropriate 3D models and materials. We evaluate our method on real photographs of indoor scenes and demonstrate the editability of the resulting scene components.

==> alt_init.tex <==
\begin{figure*}[p]
	\centering
	\small
        \setlength{\resLen}{0.9in}

	\addtolength{\tabcolsep}{-3pt}

                \begin{overpic}[height=\resLen]{img/real_3_alt/result_full.jpg}
                    \put(2, 4){\color{white} \contour{black}{(a) \textbf{Alt. Result}}}
                \end{overpic} 

        \caption{\label{fig:fig_alt}
        \ky{Our system is also robust for user to pick alternated model/texture ranked from clips search, to have different geometry and texture map for optimization} 
	}
\end{figure*}


==> pref_table.tex <==
\begin{table*}[t]
	\centering
	\small
	\caption{\label{tab:perf}
		Optimization configuration and performance statistics for our inverse-rendering results.
		All experiments are conducted on a workstation with an AMD Ryzen 9 7950X 16-core and an Nvidia RTX 4090 graphics card.
	}
	\begin{tabular}{rlrrrrrr} 
		\toprule
		%
		\multicolumn{2}{c}{\textbf{XXX}} & \textbf{\# Room} & \textbf{\# Room} & \textbf{# Geo.} & \textbf{\# Geo.} & \textbf{# Fine} & \textbf{# Fine}
		\\
		& & \textbf{Iter.} & \textbf{time} & \textbf{Iter.} &  \textbf{time} & \textbf{Iter.} & \textbf{time}
		\\
		\midrule
		Example1 & (Fig.~\ref{fig:teaser}) & 100 & 0.07s & 200 & 0.27s & 400 & 3.4s
		\\
		\bottomrule
	\end{tabular}
\end{table*}

